Physics-Infused Reduced Order Modeling of Aerothermal Loads for Hypersonic Aerothermoelastic Analysis

This paper presents a novel physics-infused reduced-order modeling (PIROM) methodology for efficient and accurate modeling of non-linear dynamical systems. The PIROM consists of a physics-based analytical component that represents the known physical processes, and a data-driven dynamical component that represents the unknown physical processes. The PIROM is applied to the aerothermal load modeling for hypersonic aerothermoelastic (ATE) analysis and is found to accelerate the ATE simulations by two-three orders of magnitude while maintaining an accuracy comparable to high-fidelity solutions based on computational fluid dynamics (CFD). Moreover, the PIROM-based solver is benchmarked against the conventional POD-kriging surrogate model, and is found to significantly outperform the accuracy, generalizability and sampling efficiency of the latter in a wide range of operating conditions and in the presence of complex structural boundary conditions. Finally, the PIROM-based ATE solver is demonstrated by a parametric study on the effects of boundary conditions and rib-supports on the ATE response of a compliant and heat-conducting panel structure. The results not only reveal the dramatic snap-through behavior with respect to spring constraints of boundary conditions, but also demonstrates the potential of PIROM to facilitate the rapid and accurate design and optimization of multi-disciplinary systems such as hypersonic structures.

==> trash/sec1_int2.tex <==
\section{Introduction} \label{sec_int}

Air-breathing hypersonic vehicles are under increasingly active development over the past decade \cite{Tzong2010, McNamara2011, Zuchowski2012, Bowcutt2018}.  Due to extreme aerothermodynamic environment at high speeds, the coupling between the structural dynamics, heat transfer, and hypersonic aerothermodynamics, viz. aerothermoelasticity (ATE), constitutes the core subsystem governing the operation of a hypersonic vehicle.  The predictive aerothermoelastic capability over extended flight time is a key ingredient for analyzing and optimizing the performance, stability, and reliability of hypersonic vehicles \cite{McNamara2011,Huang2019}.

Hypersonic aerothermoelastic analysis and design are governed by highly nonlinear time-dependent partial differential equations (PDEs) over a three-dimensional space.  More challenges arise as the highly nonlinear properties of hypersonic flow physics is accounted for in the PDEs.  For the sake of modularity and simplicity for implementation, in hypersonic ATE analysis and design, the structural, fluid and thermal domains are resolved independently, and their coupling is achieved by interfaces for information exchange \cite{Huang2019}.  However, in the pursuit of ever-higher fidelity ATE simulation of the hypersonic vehicle, the increase in the fidelity of the individual solvers typically translates to higher, sometimes intractable, computational cost.  Therefore, it has been a common practice to use reduced-order models (ROMs) as a substitution to the solver components for computational efficiency while maintaining the solution accuracy.

Most of the ROM development have focused on the aerodynamic solver, resulting in the widely-used aerothermal surrogate based on kriging regression and Proper Orthogonal Decomposition (POD), i.e. POD-kriging \cite{Falkiewicz2011, Crowell2011, Crowell2012, Huang2017a}.  However, the POD-kriging surrogate is developed for a fixed relatively simple geometrical configuration, and has generalization and characterization \cite{Huang2020a, Huang2019} issues that prohibit its practical use in ATE design and optimization of hypersonic vehicles.  Generalization pertains to the capability of the ROM to predict aerothermal loads for thermal, elastic and flow conditions, as well as geometrical configurations, different to the ones present in the training dataset.  Characterization is related the curse of dimensionality, which pertains to the intractable exponential increase in the number of training samples, as more parameters are introduced to characterize the ATE problem.  These limitations make surrogates like POD-kriging impractical for the ATE design and analysis of practical hypersonic configurations.

Several efforts have been undertaken to tackle the limitations of the aerothermal ROM, mostly using correction techniques of a certain form \cite{Crowell2011,Crowell2014,Huang2019b,Brouwer2020}.  These ROM's alleviate or partially remove the generalization and characterization issues, and have enabled the ATE optimization of hypersonic structure for specific problems \cite{Huang2020a}.  However, it would be ideal to completely remove the two issues in the aerothermal ROM's using new paradigms of machine learning (ML), to enable the multi-disciplinary design of optimization of hypersonic vehicles.

One such paradigm is known as the field inversion and machine learning (FIML) \cite{Duraisamy2016,Duraisamy2016a,Singh2017a,Singh2017,Holland2019}.  It involves the use of high-fidelity data to correct terms in a lower-fidelity model that are known to induce inaccuracies due to approximations. For example, a variety of efforts have been made on enhancing RANS predictions \cite{Ling2015,Samareh2014,Wang2017} using high-fidelity data.  In \cite{Ling2015} authors utilized high-fidelity large-eddy simulations (LES) and direct numerical simulations (DNS) data to train various machine learning models to identify regions of high RANS uncertainty driven by underlying RANS model assumptions.  Another approach to enhance RANS simulations was conducted in \cite{Wang2017}, where authors utilized DNS- and LES-trained ML models to predict Reynolds stress discrepancies in channel flows that were not present in the training data.  The successes of data-driven augmentation in RANS applications, motivate its use for ROM construction in hypersonic ATE for aerothermal load predictions.

There are two strategies for FIML implementation: the indirect and direct approaches \cite{Holland2019,Holland2019a}.  Both approaches identify the appropriate correction terms by minimizing an objective function that quantifies the difference between the augmented model and the target high-fidelity outputs.  In the indirect approach, one starts with a field inversion step.  With multiple model correctors embedded in the computational domain, an optimizer finds the optimal values of these correctors that minimize the objective.  Subsequently, in machine learning step, the field inversion data is used for offline ML training to learn the mapping functions from the input space, to the desirable values for corrections.  The most notable issues with the indirect approach is that the training features generated from the field inversion stage might not be learnable, i.e. in the machine learning stage it can be difficult to find an optimal mapping function, thus potentially diminishing the predictive capabilities of the trained model \cite{Holland2019}.  On the other hand, the direct approach integrates the steps for field inversion and machine learning.  The ML model is embedded into the objective function, and the optimization of the objective directly produces the ML model required for model augmentation.  This approach ensures that the field inversion data is learnable \cite{Holland2019a}, and has been found to enhance the generalizability of the trained models \cite{Holland2019}.  However, potential challenges in the directly approach include: 1) the high nonconvexity of the field inversion optimization attributed to the ML algorithm, 2) the computational cost of backpropagation through the ML model and ROM when conducting gradient-based optimization.

In the previous work \cite{Venegas2021}, as an attempt to resolve the issues in the aerothermal surrogates, a physics-infused reduced-order (PIRO) modeling methodology was developed.  The PIRO methodology provides a systematic procedure to augment a first-principle-based physical model with ML-based correction terms to achieve the accuracy of high-fidelity PDE-based models.  Specifically, using the indirect FIML approach, the turbulent viscous-inviscid (TVI) model \cite{Stollery1973,Brouwer2016} was augmented by correctors based on Gaussian process regression (GPR) models for the prediction of aerodynamic pressure on a deforming surface.  The augmented TVI (ATVI) model was found to be reliable for a multitude of test cases, but sometimes suffered from generalizability issues when extrapolating to thermoelastic responses that were outside the training data.  Therefore, more robust learning techniques are required to enhance the generalizability of the ATVI ROM for efficient and accurate aerothermal load predictions.

In this work, the direct FIML approach will be incorporated into the PIRO methodology to develop a new version of the ATVI model along with the most recent developments of ML models, esp. Neural Ordinary Differential Equations (NODEs) \cite{Chen2018}.  The conventional FIML methods only work with interpolative ML models, such as neural networks and GPRs, that employs an algebraic relation between the input and output.  The more recent formalism of NODE provides a dynamic, differential relation between the input and output, which are presumably able to learn more complex functional relations than the conventional ML models.  The introduction of NODE is expected to extend the PIRO methodology for generating more robust, accurate and generalizable ROMs.  In this study, the extended PIRO methodology will be used to generate the ATVI model for hypersonic aerothermal load prediction.

Specifically, the objectives of this work are:
\begin{compactenum}
    \item To integrate NODEs into the PIRO methodology with an efficient and robust gradient-based optimization implementation.
    \item To develop a new version of augmented TVI model, and assess its accuracy and computational efficiency against RANS solutions for aerothermal load predictions.
    \item To demonstrate the generalizability of the new ATVI model that enables the aerothermoelastic simulation of various different hypersonic structures.
\end{compactenum}

% The recent decade has experienced an increased interest in the development of light-weight launch hypersonic vehicles for space exploration as well as military use 
% \cite{Tzong2010, McNamara2011, Zuchowski2012, Bowcutt2018}. During the atmospheric flight, these vehicles are subjected to extreme aerothermodynamic environments that involve 
% high aerodynamic loading and heating. The thermoelastic response excited by the aerothermal loads can affect structural integrity and cause structural instabilities, such as buckling, 
% panel flutter, and control surface flutter. Therefore, the prediction of the complex flow physics is paramount for the aerothermoelastic analysis and design of light-weight hypersonic 
% structures. One of the major difficulties associated with the aerothermoelastic analysis is inherently complex hypersonic flows. At hypersonic speeds, the flow exhibits characteristics 
% such as thin shock layers, entropy layer, viscous interaction, and low-density, high-temperature flows. These are complex phenomena that require accurate and efficient modeling.

% A high-fidelity fluid solver that accounts for these highly nonlinear effects is required for capturing the essential properties of the hypersonic flow physics. Due to the high computational 
% cost of hypersonic simulations, a typical approach to resolving the panel response is through the use of surrogates and reduced order models (ROMs).  These are computationally efficient models 
% that treat the aerothermal loads as a function or an ordinary differential equation (ODE) of the flight conditions and the thermoelastic responses.  Particularly, the surrogate based on kriging 
% and Proper Orthogonal Decomposition (POD), i.e. POD-kriging, has been applied to hypersonic aerothermoelastic analysis, and accelerated the simulation by three-four orders of magnitude while
% retaining an accuracy close to the CFD solver \cite{Falkiewicz2011, Crowell2011, Crowell2012, Huang2017a}.

% The POD-kriging surrogate is essentially a regression model that treats the aerothermal loads as a function of flight conditions and the thermoelastic responses.  This type of regression model
% suffers from two fundamental limitations: generalization and characterization \cite{Huang2019,Huang2020b}.  First, the POD-kriging surrogate cannot be generalized for the aerothermal prediction 
% for the configurations, thermoelastic responses, and flow conditions that are different from those used in the training data samples.  Second, due to the curse of dimensionality, i.e. the 
% required number of training samples grows rapidly with respect to the number of inputs, it soon becomes impractical to generate aerothermal surrogates for complex hypersonic configurations, 
% where an extensive set of modes is needed to characterize the thermoelastic response.  These drawbacks of the POD-kriging surrogate have limited the existing capability to carry out the 
% multi-disciplinary design of hypersonic structures, as during the design process the configuration, thermoelastic response, and flow conditions would be all varying, and it is impractical to 
% generate new surrogates at each design iteration.

% Several correction techniques have been developed to tackle the limitations of the aerothermal surrogates \cite{Crowell2011, Crowell2014, Huang2019b}.  This type of technique starts with an
% aerothermal surrogate that is built for a reduced set of thermoelastic responses.  Subsequently, the aerothermal prediction from such a surrogate is corrected for more complex thermoelastic 
% responses using analytical or semi-empirical formulations.  The correction techniques alleviate the characterization issue by reducing the input parameters required for the thermoelastic modal
% coordinates, and thus resulting in the reduction of the number of samples \cite{Crowell2011, Crowell2014}.  Some of the correction techniques also solves the generalization issue to some
% degree by enabling the extrapolation of an aerothermal surrogate to different flight conditions, geometrical configurations, and arbitrary wall temperature distributions \cite{Huang2019b}.  
% However, the correction techniques usually work in the vicinity of the reference solution, and are not sufficiently general to enable the aerothermal prediction for \textit{arbitrary} 
%configurations and thermoelastic responses.

% There have been efforts to tackle the limitations of surrogates.  In Ref. \cite{Chen2019}, a Grassmann manifold interpolation technique is employed to construct a surrogate at a new flight condition using existing surrogates trained for other flight conditions.  However, this interpolation technique still requires a large database of surrogates for the flight conditions of interest, and cannot generalize the surrogates for different configurations.  Several correction techniques have been developed to alleviate the characterization issue of the aerothermal surrogates \cite{}.  This type of technique starts with an aerothermal solution associated with a simplified set of thermoelastic responses, and subsequently corrects the aerothermal solution for more complicated thermoelastic responses using analytical or semi-empirical formulations.  For example, in Refs. \cite{Crowell2011, Crowell2012}, an ODE-based pointwise correction scheme for heat flux was developed based on a generalized Chapman--Rubesin solution for turbulent flow over a flat surface.  This approach predicts accurately the heat flux with respect to arbitrary temperature distributions, given the thermal solution associated with a constant wall temperature.  In Refs. \cite{}, the local piston theory method was developed to correct the pressure associated with an undeformed structure to obtain the pressure on deforming structures.

% There are some emerging efforts to use alternative approaches for aerothermal load modeling, so as to circumvent the limitations in the surrogates.  In Ref. \cite{Blonigan2019}, a least-squares 
% Petrov-Galerkin ROM is developed for hypersonic flight vehicles by the projection of a high-dimensional system of RANS equations to a low-dimensional dynamical system.  This approach has less 
% constraints on the thermoelastic responses and flow conditions, however, its convergence, stability and accuracy still remain to be quantified rigorously.  In Ref. \cite{Brouwer2016}, a 
% hypersonic turbulent viscous interaction (TVI) model, based on Refs. \cite{Stollery1973}, was extended for the aerodynamic pressure prediction given the structural deformation.  
% The advantage of this approach is that the model has an accuracy comparable to high-fidelity RANS solutions, and is completely independent of the configuration, thermoelastic response, and flow
% conditions.  This means that it is particularly suitable for the multi-disciplinary design of hypersonic structures.  However, the TVI model may have numerical instability issues and there 
% lacks a systematic approach to incorporating more complex hypersonic flow physics, such as real gas effects and chemical reaction, into the formulation.

% In this work, the field inversion and machine learning (FIML) technique \cite{Ling2015, Duraisamy2016, Wang2017, Holland2019} will be employed to to obtain an augmented TVI model for robust, 
% accurate, and efficient load prediction that is suitable for aerothermoelastic analysis and design.  The FIML method is a data-driven paradigm for the augmentation of a low-fidelity model to 
% achieve an improved predictive capability that is comparable to a high-fidelity model.  The motivation of the FIML method is that, the accuracy reduction in a low-fidelity model is typically 
% due to the assumptions employed in the simplification of high-fidelity models.  It is possible to introduce new terms in the low-fidelity model, termed a closure term, to compensate for the 
% loss of accuracy due to the model simplifications.  The FIML method starts with field inversion process that determines the correct values of the closure term by comparing the low-fidelity and
% high-fidelity solutions of representative problems involving the deficient physics.  Next, a machine learning model is employed to extract the functional form of the closure term from the 
% field inversion data, which is subsequently embedded into the low-fidelity model to enhance its predictive accuracy.  The FIML method has been applied successfully to various model augmentation 
% problems, e.g. Reynolds stress modeling \cite{Wang2017}, open channel model calibration \cite{Duraisamy2016}, and separated flow prediction \cite{Holland2019}.  It was shown that the 
% FIML-augmented model demonstrates good generalization characteristics, as the predictive accuracy improves even for run cases from which data was not acquired, and geometries different to 
% those used for training \cite{Holland2019}.

%\hl{INSERT HYPATE FRAMEWORK PICTURE}

% The goal of this work is to develop an efficient and versatile hypersonic aerothermodynamic model, using an FIML-augmented TVI formulation, so as to accurately and efficiently predict pressure 
% and heat flux given arbitrary thermoelastic responses and flow conditions.  This new model will be incorporated into the HYPATE computational framework, as illustrated in 
% Fig. \ref{fig:hypate code}.  The HYPATE framework has been developed for and applied to various hypersonic aerothermoelastic problems \cite{Huang2019b,Sadagopan2020,Huang2020b}.  Subsequently,
% as a demonstration of the augmented TVI model, the enhanced framework will be employed to systematically quantify the impact of boundary layer on the aerothermoelastic response and stability 
% of typical hypersonic structures.  In our previous study \cite{Huang2019}, it has shown that a sufficiently thin boundary layer can lead to unfavorable pressure distribution and the immediate 
% onset of aerothermoelastic instability in the form of snap-through.  Therefore, the accurate understanding and modeling of the boundary layer effects on the aerothermoelastic panel response 
% is critical for the design of light-weight long-endurance hypersonic structures.

% Aeroelastic and aerothermoelastic behavior of skin panels of high speed vehicles have been studied since late 1950s \cite{Dowell1974, Mei1993}.  The theoretical and numerical studies have shown that the boundary layer has significant impact on the aeroelastic response \cite{Dowell1974, Hashimoto2009, Huang2019}, that an increasing boundary layer thickness has a beneficial effect on the flutter amplitude and a stabilizing effect on the panel by postponing the onset of instability.  However, the initial results in Ref. \cite{Huang2019} have shown that, for aerothermoelastic response, the boundary layer does not necessarily stabilize the panel in contrast to the aeroelastic case.  A sufficiently thin boundary layer can lead to unfavorable pressure distribution and the immediate onset of aerothermoelastic instability in the form of snap-through.  Therefore, the accurate understanding and modeling of the boundary layer effects on the aerothermoelastic panel response is critical for the design of light-weight long-endurance hypersonic structures.  


==> trash/sec2_piro.tex <==
\section{Physics-Infused Reduced Order Modeling}
In this section, the PIROM methodology is presented by an example. Specifically, the Tubulent Viscous-Inviscid (TVI) interactions model is subjected to the PIROM paradigm with the intent of generating an improved and efficient augmented TVI (ATVI) model. The underlying simplifications and assumptions of the physics-based ROM induce system predictions errors that significantly diminish the accuracy of the model. In this section, the physics-based TVI ROM \cite{Stollery1969,Stollery1973} is presented and subjected to the PIROM methodology. Previous work \cite{Venegas2021}, has successfully augmented the TVI equations to obtain an augmented TVI (ATVI) set of equations, which were proven to provide of high-fidelity aerothermal load predictions while maintaining the generalizable and efficient properties of the original TVI model \cite{Venegas2021}. 

\hl{The flow does not look right to me.  The flow in the extended abstract looks better.}

\subsection{Physics-Based Modeling}
The classical TVI model was originally developed in \cite{Stollery1969,Stollery1973}, and it arises as a simplification of the compressible Navier-Stokes equations with the use of several assumptions such as two-dimensional flow, constant boundary layer pressure, and freestream inviscid flow \cite{Stollery1973}. The inherent model assumptions diminishes the predictive capabilities of the model, and motivate the introduction of augmentation variables to correct for the missing physics \cite{Venegas2021}. The full description of the TVI model 
\begin{subequations}\label{eq: tvi}
    \begin{align}
        \vM(\vy,\vc;\vtt)\ddf{\vy}{x} &= \vf(\vy,\vc,x;\vu,\vtt) \label{eq: state space tvi} \\
        \vc &= \vg(\vy,x;\vu,\vtt) \label{eq: aux var}\\
        \vz &= \vh(\vy,\vc,x;\vu,\vtt) \label{eq: z}
    \end{align}
\end{subequations}

\textbf{Previous work has embedded the dynamics in algebraic form}\newline

\textbf{Present the new differential approach in this work.}\newline

\subsection{Data-Based Modeling}
After identification and augmentation of the physics-deficient terms in the ROM, the next step is properly determining the controls $\beta_H(x), \beta_C(x)$ and $\beta_W(x)$ in continuous form over the computational domain of interest. 

\textbf{Indirect Approach}\newline
In previous work, the continuous controls were extracted by a series of inverse problems, and Gaussian Process Regression (GPRs) models were used to learn the dynamics from the inverse problems data.

\textbf{Direct Approach}\newline
Write the equations in augmented system dynamics form. Identify the differential and algebraic variables. Explain the DAE nature of the problem at hand.

\subsection{Physics-Infused Modeling}

\textbf{Final description of the current implementation}\newline

